Timing Performance of the CMS High Granularity Calorimeter Prototype

This paper describes the experience with the calibration, reconstruction and evaluation of the timing capabilities of the CMS HGCAL prototype in the beam tests in 2018. The calibration procedure includes multiple steps and corrections ranging from tens of nanoseconds to a few hundred picoseconds. The timing performance is studied using signals from positron beam particles with energies between 20 GeV and 300 GeV. The performance is studied as a function of particle energy against an external timing reference as well as standalone by comparing the two different halves of the prototype. The timing resolution is found to be 60 ps for single-channel measurements and better than 20 ps for full showers at the highest energies, setting excellent perspectives for the HGCAL calorimeter performance at the HL-LHC.

==> content/3_1_TOArecoAndCalib.tex <==
\section{Reconstruction of the timing information}
\label{sec:toa_recoCalib}
%\textcolor{red}{Primary: Thorben, Review: Artur}


For every channel for which there was a sufficiently large signal there were two TDC values (TOA-rise and TOA-fall), from which two separate signal times were found. ($T_\text{rise/fall}$).  
For this corrections to the TDC values for non-linearity, time-walk and a baseline shift, that principally affected the small signals. 

The time of the signal from MCP1, corrected for time-of-flight was used to make these corrections to the TDC values, with the requirement that the signal amplitude in MCP1 was greater than 100 ADC counts, where the resolution was better than 100~ps, as shown in \ref{fig:mcpreso}.

The timing of the signals in the SKIROC2 ASIC is shown in \ref{fig:timeinformation}. There was an arbitrary, but constant, offset between the reference clock and on-chip clock (CPD) shown in the figure. As the beam was asynchronous with the clock, the distribution of signal arrival times is flat within any clock period, which can be used to measure any non-linearity in the TDC. Figure \ref{plot:TOA_calib_rise} shows the distribution of TDC values for one channel within a clock period. By fitting to this distribution we were able to extract both the non-linearity and the CPD offset for each individual channel. 

\begin{figure}[htb]
	\centering
	\includegraphics[width=0.6\linewidth]{figures/Chapter4/time_measurement.pdf}
	\caption{Timing measurements used in the calibration of the calorimeter hit timestamps. CPD denotes a arbitrary, but constant, clock-phase-difference between a given readout channel and the reference clock.}
	\label{fig:timeinformation}
\end{figure}

The time calibration of a readout channel is obtained from \ref{eq:timestampdef}.
For each channel and for the rise and fall variants separately, the expression in \ref{eq:toa_to_time} is fit to the sum of the two terms in \ref{eq:timestampdef}: the time of the signal in the MCP ($\Delta T_\text{MCP}$) and the time-of-flight (TOF) from the MCP to the readout channel's location.
%The TOF is estimated from the beam particle trajectory ($\Delta X$), reconstructed with wire chambers placed upstream of the MCP, and assuming that the shower particles proceed through the detector prototype at the speed of light ($c$).
\begin{equation}
	T~~\leftrightarrow~~\Delta T_\text{MCP}~+~TOF ~=~ \Delta T_\text{MCP}~+~\frac{\Delta X}{c}
	\label{eq:timestampdef}
\end{equation}
Only Events where 
the MCP signal amplitude is greater than \qty{100}{ADC} counts, where the MCP time is most reliable, are used.
The reference timestamps computed from the MCP and the TOF are aligned with the TOA readings in a given channel by correcting for the \qty{25}{\ns} periodicity of the digital clock, cf.~Figure~9.19a in Ref.~\cite{Quast:2020}.
In order to limit statistical uncertainties, the time calibration described below is only performed for readout channels with more than \num{1000}~hits with $E_\text{dep}\geq\qty{250}{\MIP}$ and with \num{30000} or more hits in total.
The first requirement ensures a large sample of measurements where the energy is estimated from the TOT measurement, not the ADC.
As the beam was focused on the centre of the calorimeter 
%Owing to the limited acceptance of the incident particle beam and the compactness of electromagnetic particle showers, 
only 116 readout channels, or 3\% of all channels, met these requirements.


\subsubsection{Linearization of the TOA}
\label{subsubsec:toa_lin}
We find that the non-linearity of the TOA response can be modelled using:
\begin{equation}
	\hat{f}(x | \vec{\Theta}) ~=~\Theta_1 \cdot x + \Theta_2 + \frac{\Theta_3}{x-\Theta_4}
	\label{eq:toa_tw_param}
\end{equation}
In this model, $\Theta_2$ is equivalent to calibrating out any clock-phase difference between the reference clock and the clock signal of a readout channel, labelled CPD in \ref{fig:timeinformation}.
In order to remove variations in the TOA pedestals among channels, the TOA measurements are first normalised by correcting for their pedestals ($TOA^\text{min}$) and scaling them to their full ranges ($\Delta TOA$): 
\begin{equation}
	TOA_\text{norm} ~\coloneqq~ \frac{TOA-TOA^\text{min}}{\Delta TOA}
	\label{eq:toa_norm}
\end{equation}
After normalization, \ref{eq:toa_tw_param} is fitted to the average of the (period-corrected) reference timestamps as a function of $TOA_\text{norm}$. 
The accuracy of the linearization is improved by allowing separate parameter values in the linear ($TOA_\text{norm} < 0.65$) and non-linear regions ($TOA_\text{norm} \geq 0.65$):
\begin{equation}
	f_\text{TOA}(TOA_\text{norm}) ~\coloneqq~
	\begin{cases}
		\hat{f}(TOA_\text{norm}|\vec{\Theta}_{1}^{TOA})&\text{for }TOA_\text{norm} < 0.65. \\
		\hat{f}(TOA_\text{norm}|\vec{\Theta}_{2}^{TOA})&\text{for }TOA_\text{norm} \geq 0.65.
	\end{cases}	
	\label{eq:toa_calib}
\end{equation}
The result of the linearization step is shown in \ref{plot:TOA_calib_rise} for the TOA-rise of a representative channel.
It is found that the parameterizations thus derived are consistent with the results from the first calibration results based on the asynchronous nature of the beam particles~\cite{lobanov:2020}.

\begin{figure}
% 	\captionsetup[subfigure]{aboveskip=-1pt,belowskip=-1pt}
	\centering
	\begin{subfigure}{0.325\textwidth}
% 		\centering
		\includegraphics[width=\textwidth]{plots/Chapter4/toa_calibration/toa_calib_channel32228_rise.pdf}
		\subcaption{TOA linearization, \ref{subsubsec:toa_lin}.
		\label{plot:TOA_calib_rise}
		}
	\end{subfigure}
% 	\hfill
	\begin{subfigure}{0.325\textwidth}
% 		\centering
		\includegraphics[width=\textwidth]{plots/Chapter4/hit_energy_tw_calibration/hitenergy_twchannel32228_rise.pdf}
		\subcaption{Time-walk correction, \ref{subsubsec:tw}.
		\label{plot:TW_calib_rise}
		}
	\end{subfigure}
% 	\hfill
	\begin{subfigure}{0.325\textwidth}
% 		\centering
		\includegraphics[width=\textwidth]{plots/Chapter4/module_energy_tw_calibration/moduleenergy_twchannel32228_rise.pdf}
		\subcaption{Residual correction, \ref{subsubsec:residual}.
		\label{plot:ESUMTW_calib_rise}
		}
	\end{subfigure}	
	\caption{
		The three TOA calibration steps (TOA-rise in this case) of a representative channel, centrally located inside the HGCAL prototype:
		(a) Linearization of the (normalised) TOA,
		(b) assessment of the signal-induced time-walk correction, and
		(c) assessment of the residual correction, a smaller time-walk that depends on the total energy in the module of the given channel.
		The magnitude of the time-walk corrections is about one and two orders of magnitude smaller than the calibrated time range, respectively.
	\label{plot:calibration_steps}
	}
\end{figure}


\subsubsection{Time-walk correction}
\label{subsubsec:tw}
The calibration of the signal-induced time-walk is found to also be accurately modelled using \ref{eq:toa_tw_param}.
The time-walk correction is obtained as a function of the reconstructed $E_\text{hit}$ that is used as proxy for the signal magnitude.
Therefore, the model is fit to the average of the reference timestamps corrected by $f_\text{TOA}$, as a function of $E_\text{hit}$.
The model accuracy is improved by separately fitting two regions:
where signals are reconstructed from ADC measurements ($E_\text{hit} < E_\text{TOT}$), and for larger signals reconstructed using the TOT ($E_\text{hit} \geq E_\text{TOT}$),
\begin{equation}
	f_\text{TW}(E_\text{hit}) ~\coloneqq~
	\begin{cases}
		\hat{f}(E_\text{hit}|\vec{\Theta}_{1}^{TW})&\text{for }E_\text{hit} < E_\text{TOT}. \\
		\hat{f}(E_\text{hit}|\vec{\Theta}_{2}^{TW})&\text{for }E_\text{hit} \geq E_\text{TOT}. 
	\end{cases}	
	\label{eq:toa_twcalib}
\end{equation}
As can be seen in \ref{plot:TW_calib_rise}, the time-walk is found to reach $\mathcal{O}(\qty{1}{\ns})$ for hit energies below a few \qty{100}{\MIP}.


\subsubsection{Residual time-walk correction depending on module energy}
\label{subsubsec:residual}
After correcting for the non-linearity of the TOA and its time-walk, timing inaccuracies growing to a few \qty{100}{\ps} were identified for small signals when the total energy deposited in that channel's module ($E_\text{module}$) grew larger.
It was empirically found that this residual correction can be modelled using
\begin{equation}
	f_\text{R}(E_\text{module}, E_\text{hit})~\coloneqq~
	\begin{cases}
		\mathcal{P}_4(E_\text{module})&\text{for }E_\text{hit} < E_\text{TOT}. \\
		0&\text{for }E_\text{hit} \geq E_\text{TOT}. 
	\end{cases}	
	\label{eq:toa_twmodule}
\end{equation}
In this model, $\mathcal{P}_4$ represents a fourth-degree polynomial whose parameters are determined from a fit to the average of the reference timestamps corrected by $f_\text{TOA}+f_\text{TW}$, as a function of $E_\text{module}$.
\ref{plot:ESUMTW_calib_rise} shows the residual correction determined for a representative channel.
%\newline
%\textcolor{red}{Artur: please review and improve the following explanation.}

This residual correction may in principle be due to the procedure used to estimate and subtract common-mode fluctuations~\cite{beamtest-calibration:2018} that coherently affect a large number of channels in the same module. This procedure only applies to ADC data and, therefore, to small signals.  
For larger signals, namely when $E_\text{hit}>E_\text{TOT}$, it is observed that the residual correction is negligible, as directly reflected in  \ref{eq:toa_twmodule}. For these hits, measured with the TOT, the common-mode correction does not apply, lending support to the hypothesis that the common-mode subtraction procedure may be at the root of the need for the residual correction.
While identifying the cause for this effect is beyond the scope of this work, it is suspected that the need for this residual correction is specific to the reconstruction of signals in the SKIROC2-CMS ASIC and does not necessarily generalise to other ASICs.

\subsection{Summary of the timing reconstruction}
Fitted parameter values for the example illustrated in \ref{plot:calibration_steps} are provided in \ref{table:calibconstants_fitted} of the appendix.
The fitted parameter values are found to vary by $\mathcal{O}(10\%)$ among the 116 individually time-calibrated readout channels.
Deriving and applying chip-averaged or module-averaged time calibrations for channels outside the core of electromagnetic showers has lead to an overall degradation of the combined shower performance that is discussed in \ref{sec:fullShower_perf}.
Therefore, the timing performance assessment in \ref{sec:singleChannel_perf,sec:fullShower_perf} exclusively uses the set of individually-calibrated readout channels.
These channels are located centrally in the prototype, \ie within the acceptance of electron-induced showers, as can be seen in the video-like visualization (\ref{plot:event_video_ts1,plot:event_video_ts2,plot:event_video_ts3}) of a \qty{250}{\GeV} electron showering in the time-calibrated calorimeter prototype.
\begin{figure}
% 	\captionsetup[subfigure]{aboveskip=-1pt,belowskip=-1pt}
% 	\centering
	\begin{subfigure}{0.249\textwidth}
% 		\centering
		\includegraphics[trim=58 70 67 41,clip,width=\textwidth]{plots/Chapter4/event_video/run980_event3920_ts1.pdf}
		\subcaption{$\qty{0}{\ns}\leq T\leq\qty{0.4}{\ns}$.
		\label{plot:event_video_ts1}
		}
	\end{subfigure}
% 	\hfill
    \hspace{-2mm}
	\begin{subfigure}{0.249\textwidth}
% 		\centering
		\includegraphics[trim=58 70 67 41,clip,width=\textwidth]{plots/Chapter4/event_video/run980_event3920_ts2.pdf}
		\subcaption{$\qty{0.4}{\ns}<T\leq \qty{0.8}{\ns}$.
		\label{plot:event_video_ts2}
		}
	\end{subfigure}
% 	\hfill
    \hspace{-2mm}
	\begin{subfigure}{0.249\textwidth}
% 		\centering
		\includegraphics[trim=58 70 67 41,clip,width=\textwidth]{plots/Chapter4/event_video/run980_event3920_ts3.pdf}
		\subcaption{$\qty{0.8}{\ns}<T\leq \qty{1.2}{\ns}$.
		\label{plot:event_video_ts3}
		}
	\end{subfigure}	
% 	\hfill	
    \hspace{-2mm}
	\begin{subfigure}{0.249\textwidth}
% 		\centering
		\includegraphics[trim=58 70 67 41,clip,width=\textwidth]{plots/Chapter4/event_video/run980_event3920_full.pdf}
		\subcaption{Full shower.
		\label{plot:event_video_incl}
		}
	\end{subfigure}		
	\caption{
		Time-evolution (a--c) of a \qty{250}{\GeV} electron-induced shower (d) in the HGCAL prototype.
		Data are shown for \num{81} hits with reconstructed timestamps.
		If both TOA variants are within their linear region, timestamps are computed from an average of both. 
		Otherwise, the variant in or closest to its linear region is taken.
		The size and colour of the markers both correspond to the reconstructed hit energy.
	}
\end{figure}

==> content/4_TimePerf_fullShowers_alternative.tex <==
\section{Timing performance of  the HGCAL prototype}

\textcolor{red}{\textbf{Problems with the existing draft of this section:}}
\begin{enumerate}
  \item MCP jitter too ad'hoc and inconsistently subtracted, e.g. it is for the full shower but not for the single channels
  \item Resolution-based weights include the jitter, making the argumentation more difficult
  \item Why using a resolution-weighted average at all, it is up to us on how we reconstruct the energy
  \item The analysis with expected and measured sigma in the data and MC is confusing
  \item The correlation between channels on one module should strictly speaking be part of point 3 and 4. 
  \item There is no added benefit of adding MC because the shower timestamps are instantaneous (less than one ps resolution) in the MC truth. The only discrepancy could be because of inconsistent energy distributions of hits, and in particular the number of contributing hits per shower, between data and MC. However, the MC validity in this regard is already discussed in the H3 paper.
\end{enumerate} 

\textbf{New proposed messages/scope of this section:} 
\begin{itemize}
  \item Timing resolution of single channel
  \item Timing resolution of the full CE-E prototype
  \item Establish existence of global jitter (of about 50ps) and subtract it
\end{itemize}

\textbf{Critical consequences:}
\begin{itemize}
  \item No explicit plot with MC, could say that MC reproduces our, the following findings (which it does)
  \item No resolution weighting to avoid extensive discussion on the correlation analysis
  \item (This section is much shorter, but conciser / less confusing)
\end{itemize}

\underline{The sequence of arguments could be as follows.}

\subsection{Single channel resolution}

\begin{figure}[hbtp]
  \captionsetup[subfigure]{aboveskip=-1pt,belowskip=-1pt}
  \centering
  \begin{subfigure}[b]{0.49\textwidth}
          \centering
          \includegraphics[width=0.999\textwidth]{plots/Chapter5/channel_evaluation/ref_channel69240.pdf}
          \subcaption{
          }
          \label{plot:channel_resolution}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.49\textwidth}
      \centering
      \includegraphics[width=0.999\textwidth]{plots/Chapter5/channel_vs_channel_differential/ref_channel69138.pdf}
      \caption{
      }
      \label{plot:ch_vs_ch_resolution}
  \end{subfigure}
  \caption{
  }
\end{figure}

\ref{plot:channel_resolution}:
\begin{itemize}
  \item Resolution w.r.t. MCP at 800MIPs is \SI{69}{\pico\second}, the about \SI{25}{\pico\second} MCP-MCP ("MCP intrinsic") resolution, see \ref{fig:mcpreso}, is subtracted in quadrature from this value
  \item the choice of 800 MIPs will to be kneaded in into the text. If it is "just" because it is where things plateau, this needs to be made explicit. Otherwise, one wonders about this being a meaningful energy in HGCAL. Consider the contrast with 4.2 where all the values are the asymptotic ones...
  \item All channel analysis w.r.t.: 75 plus minus 9(1) ps resolution
  \item All channel vs channel: 56 plus minus 5(1) ps (per channel)
  \item $\SI{75}{\pico\second}~\approx~\sqrt{(\sigma_{channel}^2 + \sigma_{jitter}^2 )}$
  \item Jitter is 50 plus minus 15(2) ps
\end{itemize}

\ref{plot:ch_vs_ch_resolution}:
\begin{itemize}
  \item Using one channel as a reference and assuming that the per-channel resolution does not change much beyond 800 MIPs, it holds for channels from two different modules that $\SI{79}{\pico\second}~\approx~\sqrt{2}\cdot\sigma_{channel}$. Hence, the per-channel resolution is around \SI{55}{\pico\second} for high-enough energies.
  \item The timestamps from channels on the same module are correlated (expected, affected by baseline shift /timewalk simultaneously). No need to thematise this any further.
  \item From both per-channel timing figures, it follows: $\sigma_{jitter}~\approx~(70^2 - 79^2/2)~\text{ps}~\approx~40ps$. This is of course, due to the neglect of any error-analysis, only an estimate.
\end{itemize}  


\begin{figure}[hbtp]
  \captionsetup[subfigure]{aboveskip=-1pt,belowskip=-1pt}
  \centering
  \includegraphics[width=0.49\textwidth]{plots/Chapter5/channel_evaluation/all_channel_wrt_MCP.pdf}
  \caption{
    }
  \label{plot:all_channel_resolution}
\end{figure}

\ref{plot:all_channel_resolution}:
\begin{itemize}
  \item When jitter is subtracted, resolution around 50ps
  \item Injected into MC as timestamp smearing
\end{itemize}




\subsection{Full shower resolution}


\begin{figure}[hbtp]
  \captionsetup[subfigure]{aboveskip=-1pt,belowskip=-1pt}
  \centering

  \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=0.999\textwidth]{plots/Chapter6/per_event_dt_spread/per_event_dt_wrt_mcp.pdf}
    \subcaption{
    }
    \label{plot:per_event_dt}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=0.999\textwidth]{plots/Chapter6/avg_time_event/timestamp_distribution_300GeV.pdf}
    \subcaption{
    }
    \label{plot:avg_time_event}
  \end{subfigure}  
  \caption{
  }
\end{figure}

\ref{plot:per_event_dt}:
\begin{itemize}
  \item Illustration of the existence of a global jitter w.r.t. the MCP readout system.
\end{itemize}

\ref{plot:avg_time_event}:
\begin{itemize}
  \item Full shower timestamp (computer from energy-weighted sum) w.r.t. MCP resolution is about \SI{57}{\pico\second}, intrinsic MCP resolution is already subtracted in quadrature: $\SI{57}{\pico\second}~\approx~\sqrt{(\sigma_{jitter}^2+\sigma_{HGC}^2)}$
  \item Odd vs. even layer shower timestamp resolution is about \SI{36}{\pico\second}. Assuming that the timing resolution of half the prototype (neighboring even and odd layers have approximately same distribution of deposited energy) is $\sqrt(2)$x the full prototype's resolution: $\SI{36}{\pico\second}~\approx~2\cdot\sigma_{HGC}$.
  \item Solving for the jitter term: $\sigma_{jitter}~=~\sqrt{(57^2-(36/2)^2)}~\text{ps}~\approx~\SI{54}{\pico\second}$, in reasonable agreement with the estimate from the per-channel example above.
  \item Consistent picture from all beam energies. Combined result is 53.1 plus minus 0.3 ps!
  \item This estimate incorporates proper error propagation and is the reliable estimate of the jitter contribution.
\end{itemize}

\begin{figure}[hbtp]
  \captionsetup[subfigure]{aboveskip=-1pt,belowskip=-1pt}
  \centering
  \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=0.999\textwidth]{plots/Chapter6/shower_timing_bias_resolution/bias.pdf}
    \subcaption{
      }
      \label{plot:shower_bias}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.49\textwidth}
      \centering
      \includegraphics[width=0.999\textwidth]{plots/Chapter6/shower_timing_bias_resolution/resolution.pdf}
      \subcaption{
      }
      \label{plot:shower_resolution}
  \end{subfigure}
    \caption{
  }
\end{figure}

\ref{plot:shower_bias}:
\begin{itemize}
  \item 50 MIPs onward
  \item Full-shower (energy weighting) bias w.r.t. MCP. MCP assumed to have zero bias w.r.t. true incidence --> bias is less than \SI{20}{\pico\second} over tested energy range.
\end{itemize}

\ref{plot:shower_resolution}:
\begin{itemize}
  \item The ultimate resolution figure, with the MCP contribution subtracted --> 16 ps!!!.
  \item By the way, 16ps is also what one obtains as the expected sigma from MC, using the per-channel resolution with the jitter subtracted. This could be a good closure check to have available during the reviewing if necessary.
\end{itemize}


\begin{figure}[hbtp]
  \captionsetup[subfigure]{aboveskip=-1pt,belowskip=-1pt}
  \centering
  \includegraphics[width=0.49\textwidth]{plots/Chapter6/shower_timing_bias_resolution/resolution_vs_nmips.pdf}
  \caption{
    }
  \label{plot:resolution_nhits}
\end{figure}

\ref{plot:resolution_nhits}:
\begin{itemize}
  \item Resolution as function of hit selection threshold
  \item For highest energy to probe relevant hit energy range
\end{itemize}


\textcolor{red}{To add: add MC in the last two figures}
